Top-k Training of GANs: Improving GAN Performance by Throwing Away Bad Samples

We introduce a simple (one line of code) modification to the Generative Adversarial Network (GAN) training algorithm that materially improves results with no increase in computational cost: When updating the generator parameters, we simply zero out the gradient contributions from the elements of the batch that the critic scores as `least realistic'. Through experiments on many different GAN variants, we show that this `top-k update' procedure is a generally applicable improvement. In order to understand the nature of the improvement, we conduct extensive analysis on a simple mixture-of-Gaussians dataset and discover several interesting phenomena. Among these is that, when gradient updates are computed using the worst-scoring batch elements, samples can actually be pushed further away from their nearest mode. We also apply our method to recent GAN variants and improve state-of-the-art FID for conditional generation from 9.21 to 8.57 on CIFAR-10.

==> our_figures/mog_figs.tex <==
%\begin{figure}[t]
%    \begin{subfigure}[c]{0.5\textwidth}
%        \centering
%        \includegraphics[width=1\linewidth]{our_figures/bottomk_cosine.png}
%    \end{subfigure}
%    \begin{subfigure}[c]{0.5\textwidth}
%        \centering
%        \includegraphics[width=1\linewidth]{our_figures/bottomk_distance.png}
%    \end{subfigure}
%    \begin{subfigure}[c]{0.5\textwidth}
%        \centering
%        \includegraphics[width=1\linewidth]{our_figures/our_cosine.png}
%    \end{subfigure}
%    \begin{subfigure}[c]{0.5\textwidth}
%        \centering
%        \includegraphics[width=1\linewidth]{our_figures/our_distance.png}
%    \end{subfigure}
%    \caption{Evaluation of influential DML model parameters and architectures on the CUB200-2011 and CARS196 dataset.}
%    \label{fig:ablation_studies}
%\end{figure}

\begin{figure*}
    \centering     %%% not \center
    \subfigure[Cosine Similarity with Top-$k$]{\includegraphics[width=0.35\linewidth]{our_figures/our_cosine.png}}
    \subfigure[Cosine Similarity with Bottom-$k$]{\includegraphics[width=0.35\linewidth]{our_figures/bottomk_cosine.png}}
    \subfigure[Distance to nearest mode with Top-$k$]{\includegraphics[width=0.35\linewidth]{our_figures/our_distance.png}}
    \subfigure[Distance to nearest mode with Bottom-$k$]{\includegraphics[width=0.35\linewidth]{our_figures/bottomk_distance.png}}
    \caption{my caption}
\end{figure*}
